Lessons learned from the evaluation of Spanish Language Models

Given the impact of language models on the field of Natural Language Processing, a number of Spanish encoder-only masked language models (aka BERTs) have been trained and released. These models were developed either within large projects using very large private corpora or by means of smaller scale academic efforts leveraging freely available data. In this paper we present a comprehensive head-to-head comparison of language models for Spanish with the following results: (i) Previously ignored multilingual models from large companies fare better than monolingual models, substantially changing the evaluation landscape of language models in Spanish; (ii) Results across the monolingual models are not conclusive, with supposedly smaller and inferior models performing competitively. Based on these empirical results, we argue for the need of more research to understand the factors underlying them. In this sense, the effect of corpus size, quality and pre-training techniques need to be further investigated to be able to obtain Spanish monolingual models significantly better than the multilingual ones released by large private companies, specially in the face of rapid ongoing progress in the field. The recent activity in the development of language technology for Spanish is to be welcomed, but our results show that building language models remains an open, resource-heavy problem which requires to marry resources (monetary and/or computational) with the best research expertise and practice.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	//
Acknowledgments	main.tex	/^\\section*{Acknowledgments}$/;"	s
Agerri2020ProjectingHA	references.bib	/^@inproceedings{Agerri2020ProjectingHA,$/;"	j
Aghajanyan2021BetterFB	references.bib	/^@inproceedings{Aghajanyan2021BetterFB,$/;"	j
Agirre2014SemEval2014T1	references.bib	/^@inproceedings{Agirre2014SemEval2014T1,$/;"	j
Agirre2015SemEval2015T2	references.bib	/^@inproceedings{Agirre2015SemEval2015T2,$/;"	j
Artetxe2022DoesCQ	references.bib	/^@inproceedings{Artetxe2022DoesCQ,$/;"	j
BERTIN	references.bib	/^@article{BERTIN,$/;"	a
Better research reporting practices should be encouraged.	main.tex	/^\\paragraph{Better research reporting practices should be encouraged.} The$/;"	P	section:Discussion
Bhattacharjee2021BanglaBERTCE	references.bib	/^@inproceedings{Bhattacharjee2021BanglaBERTCE,$/;"	j
CaneteCFP2020	references.bib	/^@inproceedings{CaneteCFP2020,$/;"	j
Clark2020ELECTRAPT	references.bib	/^@inproceedings{Clark2020ELECTRAPT,$/;"	j
Comparison to the state-of-the-art.	main.tex	/^\\paragraph{Comparison to the state-of-the-art.} In relation to the previous$/;"	P	section:Discussion
Conclusion	main.tex	/^\\section{Conclusion}$/;"	s
Conneau2018XNLIEC	references.bib	/^@inproceedings{Conneau2018XNLIEC,$/;"	j
Conneau2020UnsupervisedCR	references.bib	/^@inproceedings{Conneau2020UnsupervisedCR,$/;"	j
DBLP	references.bib	/^@inproceedings{DBLP:conf\/evalita\/EspinosaARC20,$/;"	j
DBLP	references.bib	/^@inproceedings{DBLP:journals\/corr\/abs-1908-07448,$/;"	j
Devlin19	references.bib	/^@inproceedings{Devlin19,$/;"	j
Discussion	main.tex	/^\\section{Discussion}\\label{sec:discussion}$/;"	s
Experimental setup	main.tex	/^\\section{Experimental setup}\\label{sec:experimental-setup}$/;"	s
He2021DeBERTaV3ID	references.bib	/^@inproceedings{He2021DeBERTaV3ID,$/;"	j
Introduction	main.tex	/^\\section{Introduction}$/;"	s
Is there an explanation for the lower performance of some models?	main.tex	/^\\paragraph{Is there an explanation for the lower performance of some models?}$/;"	P	section:Discussion
Komatsuzaki2019OneEI	references.bib	/^@inproceedings{Komatsuzaki2019OneEI,$/;"	j
Lai2019BridgingTD	references.bib	/^@inproceedings{Lai2019BridgingTD,$/;"	j
Lai2020	references.bib	/^@article{Lai2020,$/;"	a
Liu2019RoBERTaAR	references.bib	/^@inproceedings{Liu2019RoBERTaAR,$/;"	j
Models details	main.tex	/^\\subsection{Models details}\\label{sec:model-details}$/;"	u	section:Spanish Language models
Mohtarami2018	references.bib	/^@InProceedings{Mohtarami2018,$/;"	j
MultiAzterTest	references.bib	/^@inproceedings{MultiAzterTest,$/;"	j
Nozza2020WhatT	references.bib	/^@inproceedings{Nozza2020WhatT,$/;"	j
Nzeyimana2022KinyaBERTAM	references.bib	/^@inproceedings{Nzeyimana2022KinyaBERTAM,$/;"	j
OrtizSuarezSagotRomary2019	references.bib	/^@inproceedings{OrtizSuarezSagotRomary2019,$/;"	j
Otegi2020ConversationalQA	references.bib	/^@inproceedings{Otegi2020ConversationalQA,$/;"	j
Pires2019HowMI	references.bib	/^@inproceedings{Pires2019HowMI,$/;"	j
PolignanoEtAlCLIC2019	references.bib	/^@InProceedings{PolignanoEtAlCLIC2019,$/;"	j
Related Work	main.tex	/^\\section{Related Work}\\label{sec:related-work}$/;"	s
Results	main.tex	/^\\section{Results}\\label{sec:results}$/;"	s
SLON2017-Stance	references.bib	/^@inproceedings{SLON2017-Stance,$/;"	j
SQYQP	references.bib	/^@inproceedings{SQYQP,$/;"	j
SanchezBayona2022LeveragingAN	references.bib	/^@inproceedings{SanchezBayona2022LeveragingAN,$/;"	j
Sang2002IntroductionTT	references.bib	/^@inproceedings{Sang2002IntroductionTT,$/;"	j
Schwenk2018ACF	references.bib	/^@inproceedings{Schwenk2018ACF,$/;"	j
Spanish Language models	main.tex	/^\\section{Spanish Language models}\\label{sec:spanish-language-models}$/;"	s
Straka2019EvaluatingCE	references.bib	/^@inproceedings{Straka2019EvaluatingCE,$/;"	j
Tanvir2021EstBERTAP	references.bib	/^@inproceedings{Tanvir2021EstBERTAP,$/;"	j
Taul2008AnCoraMA	references.bib	/^@inproceedings{Taul2008AnCoraMA,$/;"	j
Tiedemann2020OPUSMTB	references.bib	/^@inproceedings{Tiedemann2020OPUSMTB,$/;"	j
Training a monolingual model, is it worth it?	main.tex	/^\\paragraph{Training a monolingual model, is it worth it?}  Common wisdom$/;"	P	section:Discussion
Virtanen2019MultilingualIN	references.bib	/^@inproceedings{Virtanen2019MultilingualIN,$/;"	j
Vries2019BERTjeAD	references.bib	/^@inproceedings{Vries2019BERTjeAD,$/;"	j
Vychegzhanin2019	references.bib	/^@article{Vychegzhanin2019,$/;"	a
What should be the next steps for Spanish models?	main.tex	/^\\paragraph{What should be the next steps for Spanish models?} One could argue$/;"	P	section:Discussion
Which model should I use according to my computing budget?	main.tex	/^\\paragraph{Which model should I use according to my computing budget?} If the$/;"	P	section:Discussion
Which model should I use according to my task?	main.tex	/^\\paragraph{Which model should I use according to my task?} In this work we$/;"	P	section:Discussion
Wolf2019TransformersSN	references.bib	/^@inproceedings{Wolf2019TransformersSN,$/;"	j
WordUp	references.bib	/^@inproceedings{WordUp,$/;"	j
Wu2020AreAL	references.bib	/^@inproceedings{Wu2020AreAL,$/;"	j
Yang2019PAWSXAC	references.bib	/^@inproceedings{Yang2019PAWSXAC,$/;"	j
Zamorano2020OverviewOC	references.bib	/^@inproceedings{Zamorano2020OverviewOC,$/;"	j
agerri-etal-2020-give	references.bib	/^@inproceedings{agerri-etal-2020-give,$/;"	j
akbik-etal-2018-contextual	references.bib	/^@inproceedings{akbik-etal-2018-contextual,$/;"	j
armengol-estape-etal-2021-multilingual	references.bib	/^@inproceedings{armengol-estape-etal-2021-multilingual,$/;"	j
baly-etal-2018-integrating	references.bib	/^@inproceedings{baly-etal-2018-integrating,$/;"	j
basile-etal-2019-semeval	references.bib	/^@inproceedings{basile-etal-2019-semeval,$/;"	j
bloom	references.bib	/^@inproceedings{bloom,$/;"	j
bradley1999affective	references.bib	/^@techreport{bradley1999affective,$/;"	t
cignarella2020sardistance	references.bib	/^@InProceedings{cignarella2020sardistance,$/;"	j
dellaposta2015	references.bib	/^@article{dellaposta2015,$/;"	a
derczynski-etal-2017-semeval	references.bib	/^@inproceedings{derczynski-etal-2017-semeval,$/;"	j
evrard-EtAl	references.bib	/^@InProceedings{evrard-EtAl:2020:LREC,$/;"	j
fasttext1_bojanowski2017enriching	references.bib	/^@article{fasttext1_bojanowski2017enriching,$/;"	a
firstpage	main.tex	/^\\label{firstpage} \\maketitle$/;"	l
friedman2001greedy	references.bib	/^@article{friedman2001greedy,$/;"	a
gorrell-etal-2019-semeval	references.bib	/^@inproceedings{gorrell-etal-2019-semeval,$/;"	j
gpt3	references.bib	/^@inproceedings{gpt3,$/;"	j
gutierrezfandino2022	references.bib	/^@article{gutierrezfandino2022,$/;"	a
iberlef2021	references.bib	/^ @inproceedings{iberlef2021,$/;"	j
karthikeyan2020cross	references.bib	/^@inproceedings{karthikeyan2020cross,$/;"	j
kiesel-etal-2019-semeval	references.bib	/^@inproceedings{kiesel-etal-2019-semeval,$/;"	j
kreutzer-etal-2022-quality	references.bib	/^@article{kreutzer-etal-2022-quality,$/;"	a
kuccuk2020stance	references.bib	/^@article{kuccuk2020stance,$/;"	a
martin-etal-2020-camembert	references.bib	/^@inproceedings{martin-etal-2020-camembert,$/;"	j
mikolov2013distributed	references.bib	/^@inproceedings{mikolov2013distributed,$/;"	j
mohammad-etal-2016-semeval	references.bib	/^@inproceedings{mohammad-etal-2016-semeval,$/;"	j
montefinese2014adaptation	references.bib	/^@article{montefinese2014adaptation,$/;"	a
opt	references.bib	/^@inproceedings{opt,$/;"	j
russell1980circumplex	references.bib	/^@article{russell1980circumplex,$/;"	a
sec:discussion	main.tex	/^\\section{Discussion}\\label{sec:discussion}$/;"	l
sec:experimental-setup	main.tex	/^\\section{Experimental setup}\\label{sec:experimental-setup}$/;"	l
sec:model-details	main.tex	/^\\subsection{Models details}\\label{sec:model-details}$/;"	l
sec:related-work	main.tex	/^\\section{Related Work}\\label{sec:related-work}$/;"	l
sec:results	main.tex	/^\\section{Results}\\label{sec:results}$/;"	l
sec:spanish-language-models	main.tex	/^\\section{Spanish Language models}\\label{sec:spanish-language-models}$/;"	l
t5	references.bib	/^@article{t5,$/;"	a
tab:mod-results	main.tex	/^\\label{tab:mod-results}$/;"	l
tab:result	main.tex	/^\\label{tab:result}$/;"	l
tab:spanish-lm	main.tex	/^\\label{tab:spanish-lm}$/;"	l
taule2018overview	references.bib	/^@inproceedings{taule2018overview,$/;"	j
thorne-etal-2018-fever	references.bib	/^@inproceedings{thorne-etal-2018-fever,$/;"	j
urbizu-etal-2022-basqueglue	references.bib	/^@inproceedings{urbizu-etal-2022-basqueglue,$/;"	j
vaswani2017attention	references.bib	/^@inproceedings{vaswani2017attention,$/;"	j
wang-etal-2021-automated	references.bib	/^@inproceedings{wang-etal-2021-automated,$/;"	j
xue-etal-2021-mt5	references.bib	/^@inproceedings{xue-etal-2021-mt5,$/;"	j
zheng-etal-2021-allocating	references.bib	/^@inproceedings{zheng-etal-2021-allocating,$/;"	j
zotova2021semi	references.bib	/^@article{zotova2021semi,$/;"	a

